A FETI approach to domain decomposition for meshfree discretizations of nonlocal problems

We propose a domain decomposition method for the efficient simulation of nonlocal problems. Our approach is based on a multi-domain formulation of a nonlocal diffusion problem where the subdomains share "nonlocal" interfaces of the size of the nonlocal horizon. This system of nonlocal equations is first rewritten in terms of minimization of a nonlocal energy, then discretized with a meshfree approximation and finally solved via a Lagrange multiplier approach in a way that resembles the finite element tearing and interconnect method. Specifically, we propose a distributed projected gradient algorithm for the solution of the Lagrange multiplier system, whose unknowns determine the nonlocal interface conditions between subdomains. Several two-dimensional numerical tests illustrate the strong and weak scalability of our algorithm, which outperforms the standard approach to the distributed numerical solution of the problem. This work is the first rigorous numerical study in a two-dimensional multi-domain setting for nonlocal operators with finite horizon and, as such, it is a fundamental step towards increasing the use of nonlocal models in large scale simulations.

==> Implementation.tex <==
\section{Implementation}\label{sec:implementation}

\begin{algorithm}
    \For{each processor $i$}{
    \emph{assemble local matrices $A_i,F_i,M_i,Z_i$ and local preconditioner $N_i$}\;
    $g_{i} = Z_i^T F_i, \quad e_{i} = M_i A^\dagger_i F_i$\;
    }
    
    
    
    \If{ processor 0}{
    \emph{assemble global matrices $M,Z$, construct global projection matrix $P$};\
    }
    
    \For{each processor $i$}{
    \emph{Calculate distributed initial guess }$\lambda_i \doteq G_i(G^\intercal G)^\dagger_i g_i $
    $x_i \doteq M_i A_i^\dagger M_i^T \lambda_i,\quad z_i = N_i r_i, \quad y_i = P_iz_i, \quad p_i = y_i;$
    }
    \Repeat{$r^T y$ is small enough}{
    \For{each processor $i$}{
    $x_i = M_i A_i^\dagger M_i^T p,\quad x_i \doteq P_i x_i$\
    
    $r^+_i = r_i - \frac{r_i^T y_i}{p_i^T x_i} p_i, \quad \lambda_i = \lambda_i + \frac{r_i^T y_i}{p_i^T x_i} p_i $\ 
    
    $z_i =N_i r_i^+, y_i^+ \doteq P_i z_i \quad p_i = y_i^+ + \frac{(r_i^+)^T y_i^+}{r_i^T y_i}p_i$\
    
    $y_i \leftarrow y_i^+, \quad r_i\leftarrow r_i^+ $
    }
    }
    \caption{Projected CG}
    \label{algo:parallelAlgorithm}
\end{algorithm}



\begin{algorithm}
    \For{each processor $i$}{
    \emph{assemble local matrices $A_i,F_i,M_i,Z_i$}\;
    $g_{i} = Z_i^T F_i, \quad e_{i} = M_i A^\dagger_i F_i$\;
    }
    
    \If{ processor 0}{
    \emph{assemble global matrices $M,Z$, construct global projection matrix $P$ and preconditioner $N$};\
    
    $e = \textrm{Reduce}(e_i,\textrm{sum}), \quad g =\textrm{Reduce}(g_i,\textrm{sum}) $\;
    \emph{broadcast initial guess }$\lambda = G(G^T G)^\dagger g $
    }
    \For{each processor $i$}{
    $x_i = M_i A_i^\dagger M_i^T \lambda$\;
    }
    \If{processor 0}{
    $x = \textrm{Reduce}(x_i,\textrm{sum}),\quad r = e - x, \quad r\leftarrow Pr$\ 
    
    $z = Nr, \quad y=Pz, \quad p =y, \quad$ \emph{broadcast $p$} 
    }
    \Repeat{$r^T y$ is small enough}{
    \For{each processor $i$}{
    $x_i = M_i A_i^\dagger M_i^T p$\;
    }
    \If{processor 0}{
    $x = \textrm{Reduce}(x_i,\textrm{sum}),\quad x \leftarrow Px$\
    
    $r^+ = r - \frac{r^T y}{p^T x} p, \quad \lambda \leftarrow \lambda + \frac{r^T y}{p^T x} p $\ 
    
    $z =Nr^+, y^+=Pz$\
    
    \Repeat{$\max_{j}\{ \frac{(G^j)^T y^+ }{ \norm{G^j} \norm{y^+} }  \}$ is small enough }{
    $y^+ \leftarrow Py^+$
    }
    
    $y \leftarrow y^+, \quad r\leftarrow r^+, \quad p \leftarrow y^+ + \frac{(r^+)^T y^+}{r^T y}p, \quad$ \emph{broadcast $p$}
    }
    }
    \caption{Projected CG with iterative refinement}
    \label{algo:parallelAlgorithm}
\end{algorithm}


\begin{algorithm}
    \caption{Fully distributed projected CG with iterative refinement}
    \label{algo:parallelAlgorithm}
\end{algorithm}
